Starker Effekt von Schnelltests (Strong effect of rapid tests)

This article is a reproduction of a Fraunhofer ITWM report from 28 June 2021 on the contribution of various non-pharmaceutical measures in breaking the 3rd Corona wave in Germany. The main finding is that testing contributed more to the containment of the pandemic in this phase than vaccination or contact restrictions. The analysis is based on a new epidemiological cohort model that represents testing, vaccination and contact restrictions by time-varying rates of detection, vaccination and contacts, respectively. Only the effectiveness of different vaccines is taken from the literature. All other parameters are automatically identified in such a way that the simulated and the published incidences and death rates match. Among these parameters are incubation time, mean duration of the infectious phase, mortality rate, as well as two contact rates and one detection rate per week. Note that we can reconstruct such a high number of parameters only because we assume that the weekly wave patterns in new infections follow real infection dynamics, periodically driven by high contact rates on weekdays and lower ones on weekends. Usually, people assume that the weekly wave patterns are just reporting artefacts and that weekly mean values are the finest usable data. One focus of the paper is to quantify the increase in detection rate due to the introduction of rapid testing in schools. For this purpose, we compare federal states that differ in the start of school tests and Easter holidays. There is a clear temporal correlation with the identified detection rates. Finally, we compare the effect of the individual non-pharmaceutical measures by replacing one by one the fitted rates of detection, vaccination and contacts by neutral ones. The increase in the simulated number of actually infected persons measures the effect of the measure ignored.

==> tables/parameters0.tex <==
\begin{table}[!h]
  \centering
  \begin{tabular}{clrl}
    \hline \noalign{\smallskip}
     Symbol & Bedeutung & \multicolumn{1}{l}{Wert} & Einheit \\
    \hline \noalign{\smallskip}
    $t_0$ & Start der Simulation & 7.3.2020 0:00 & \\
    $t_1$ & Ende der Simulation & 4.5.2020 0:00 & \\
    $G$ & Zahl der Mitglieder& $83.17 \times 10^6$ & p \\
    $\tau^s$ & Beginn der infektiösen Phase & $5.9\pm0.08$ & d \\
    $\tau^e\!-\!\tau^s$ & Dauer der infektiösen Phase & $1.58\pm0.14$ & d \\
    $\tau^d$ & Zeit von Ansteckung bis Meldung bei Entdeckung & $13.86\pm0.09$ & d\\
    $\tau^l$ & Zeit von Ansteckung bis Tod bei Tod & $26.71\pm0.16$ & d\\
    $\mu$ & Anteil der Infizierten, die in der Folge sterben.& $1.14\pm0.01$ & \%\\
    $\lambda$ & Anteil der Infizierten, die entdeckt werden. & $25$ & \% \\
    $N^0$ & Vorfaktor exponentieller Verlauf vor Start & $77696\pm1448$ & p \\
    $\alpha$ & Zeitfaktor exponentieller Verlauf vor Start & $0.247\pm0.004$ & 1/d \\
    \noalign{\smallskip}
    \hline
  \end{tabular}
  \caption{Modellparameter.}
  \label{tab:fruehjahr:Modellparameter}
\end{table}


==> tables/reproduction0.tex <==
\begin{table}[!h]
  \centering
  \begin{tabular}{p{0.3 \textwidth}rrr}
    \hline \noalign{\smallskip}
    Ereignis & \multicolumn{1}{l}{Beginn} & Sprungversatz [d] & Reproduktionszahl \\
    \hline \noalign{\smallskip}
    ohne Maßnahme & & & $ 2.68 \pm 0.48 $\\
    Ende Großereignisse &  8.3.2020 & 0.00 & $ 1.66 \pm 0.08 $\\
    Reisebeschränkungen \& Schließungen & 17.3.2020 & -1.20 & $ 1.09 \pm 0.04 $\\
    Kontaktbeschränkungen & 22.3.2020 & 0.87 & $ 0.79 \pm 0.03 $\\
    - & 29.3.2020 & -0.04 & $ 0.53 \pm 0.05 $\\
    Anfang Karwoche &  5.4.2020 & -3.04 & $ 0.75 \pm 0.03 $\\
    Ostersonntag & 12.4.2020 & 0.01 & $ 0.64 \pm 0.07 $\\
    \noalign{\smallskip}
    \hline
  \end{tabular}
  \caption{Reproduktionszahl.}
  \label{tab:fruehjahr:Reproduktionszahl}
\end{table}

